Statistical Inference for Misspecified Contextual Bandits

Contextual bandit algorithms have transformed modern experimentation by enabling real-time adaptation for personalized treatment. Yet these advantages create challenges for statistical inference due to adaptivity. We study inference with contextual-bandit data without assuming a well-specified outcome model. In this setting, we show a previously overlooked issue: standard algorithms such as LinUCB may fail to stabilize under misspecified working models, leading to non-Gaussian estimator behavior and invalid inference. This issue is practically important, as misspecified working models -- such as approximations of complex dynamical systems -- are often employed by online agents in real-world adaptive experiments to balance reward, computational tractability, and robustness. We develop an inverse-probability-weighted Z-estimation framework for a broad class of marginal moment targets, including projection parameters, structural parameters with noisy contexts, and off-policy values. We identify a stability condition tailored to this framework, scaled inverse-propensity convergence, under which the IPW-Z estimator is consistent and asymptotically normal with a consistent sandwich variance estimator. We further establish sufficient conditions for scaled inverse-propensity convergence for several policy classes, including multi-armed bandit algorithms and smooth contextual allocation policies. Simulations and a HeartSteps V1 real-data-calibrated application show reliable coverage and competitive performance across multiple targets. Overall, our results highlight the importance of stability-aware adaptive design for valid post-experiment inference.

==> mystyle.tex <==
%-----------------------------------------------------------------%
%
% The latex macro
%
%-----------------------------------------------------------------%

\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsthm}
\RequirePackage{bm}
\RequirePackage{url}
\usepackage{multirow}
%\usepackage{natbib}
\usepackage{graphicx}
\usepackage{subfig}  % was: subfigure (deprecated, not installed on this machine)
%\usepackage{makecell}  % disabled: not installed locally; no \makecell/\thead used
\usepackage{booktabs}
\usepackage{array}
\usepackage{url}
\usepackage{algorithm}
\usepackage{algorithmic}
%\usepackage{dsfont}  % disabled: not installed locally. \mathds{1} fallback below.
\providecommand{\mathds}[1]{\mathbb{#1}}  % fallback shim for \mathds{1}
\usepackage{mathtools}
%\usepackage{xcolor}
%\usepackage[title]{appendix}  % disabled: not installed; fallback below
% Fallback: re-declare `appendix` as an environment that switches to \appendix
% mode. The built-in \appendix is a command; we save it then free the macro
% before declaring the environment of the same name.
\providecommand{\appendixname}{Appendix}
\makeatletter
\let\@builtinappendix\appendix
\let\appendix\relax
\newenvironment{appendix}{\par\@builtinappendix}{\par}
\makeatother

% Comments
\usepackage{xcolor}
\newcount\comments  % 0 suppresses notes to selves in text
\comments=1  % TODO: change to 0 for final version
\newcommand{\genComment}[2]{\ifnum\comments=1{\textcolor{#1}{\textsf{\footnotesize #2}}}\fi}
\newcommand{\ambuj}[1]{\genComment{red}{[AT:#1]}}
\newcommand{\ziping}[1]{\genComment{green}{[ZP:#1]}}
\newcommand{\tarun}[1]{\genComment{blue}{[TG:#1]}}
\newcommand{\YG}[1]{\genComment{purple}{[YG:#1]}}


% -------- New Packages -------- %
\usepackage{enumitem}

%------ kpfonts -------%
%\usepackage{kpfonts}

%------- some other packages -------%
\usepackage{enumerate}
% \usepackage[OT1]{fontenc}
%\usepackage{natbib}
% \usepackage[usenames]{color}
%\usepackage[dvips]{graphicx}
%\usepackage[protrusion=true, expansion=true, tracking=true, spacing=true, final, babel]{microtype}
%\usepackage{makecell}
% \usepackage[colorlinks,
% linkcolor=blue,
% anchorcolor=blue,
% citecolor=blue
% ]{hyperref}
% \usepackage{hyperref}

%\usepackage{refcheck}

\usepackage{mathrsfs}
% \usepackage{fullpage}

%--------- new defs --------%



\def\TV{\mathop{\text{TV}}}
\def\supp{\mathop{\text{supp}}}
\def\card{\mathop{\text{card}}}
\def\rank{\mathrm{rank}}
\long\def\comment#1{}
\def\skeptic{{\sc skeptic}}
\def\NPN{\bPiox{\it NPN}}
\def\vec{\mathop{\text{vec}}}
\def\dr{\displaystyle \rm}
\def\OLS{\mathop{\text{OLS}}}
\def\ts{\textstyle}
\def\skeptic{{\sc skeptic}}
\providecommand{\bnorm}[1]{\Big\vvvert#1\Big\vvvert}
\providecommand{\norm}[1]{\vvvert#1\vvvert}
\def \txb {\overbar{\xb}}
\def \tx {\overbar{x}}

\def\bess{\bes\small }
\def\Shat{{\widehat S}}
\def\lam{\rho}
\def\real{{\mathbb{R}}}
\def\R{{\real}}
\def\Ti{T_{\rm init}}
\def\Tm{T_{\rm main}}
\def\bcdot{{\bm \cdot}}
\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\cIs}{\cI_{\hat{s}}}
\def \hbeta {\widehat{\beta}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing


\newcommand{\dimq}{m_q}

\renewcommand{\baselinestretch}{1.1}

\def\sep{\;\big|\;}
\newcommand{\chz}[1]{{\textcolor{red}{[CHZ: #1]}}}
\newcommand{\hf}[1]{{\textcolor{red}{[FH: #1]}}}
\def \trunc{\mathop{\text{trunc}}}
\def \obs {{\rm obs}}
\def \mis {{\rm mis}}
\def \hbSigma {\widehat{\bSigma}}
\def \bbSigma {\bar{\bSigma}}


\newcommand{\tcT}{\tilde{\cT}}


%\usepackage[protrusion=false,expansion=true]{microtype}
%\usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}


\def\##1\#{\begin{align}#1\end{align}}
\def\$#1\${\begin{align*}#1\end{align*}}

\let\cite\citet


\let\hat\widehat
\let\tilde\widetilde
\let\check\widecheck
\def\given{{\,|\,}}
\def\biggiven{{\,\big|\,}}
\def\Biggiven{{\,\Big|\,}}
\def\bigggiven{{\,\bigg|\,}}
\def\Bigggiven{{\,\Bigg|\,}}
\def\ds{\displaystyle}
\newcommand\wtilde{\stackrel{\sim}{\smash{\mathcal{W}}\rule{0pt}{1.1ex}}}



\newcommand{\eqal}[1]{\begin{equation}\begin{aligned} #1 \end{aligned}\end{equation}}
\newcommand{\bbr}[1]{\left[ {#1} \right]}
\newcommand{\bpa}[1]{\left( {#1} \right)}
\newcommand{\E}[1]{\textbf{E} \left[ {#1} \right]}
\newcommand{\pr}[1]{\textbf{P} \left({#1}\right)}
\newcommand{\nrm}[2]{\left \lVert {#2} \right \rVert_{#1}}


%----- bold fonts -----%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
\newcommand{\bbf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bi}{\bmf{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bbm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}




\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}


%----- calligraphic fonts -----%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}


\newcommand{\sB}{\mathscr{B}}



%----- blackboard bold fonts-----%

\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\OOmega}{\mathbb{\Omega}}




%----- bold greek fonts -----%

\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\bvarepsilon}{\bm{\varepsilon}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\bm{\vartheta}}
\newcommand{\bkappa}{\bm{\kappa}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bnu}{\bm{\nu}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\bvarpi}{\bm{\varpi}}
\newcommand{\brho}{\bm{\varrho}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\bvarsigma}{\bm{\varsigma}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bupsilon}{\bm{\upsilon}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bvarphi}{\bm{\varphi}}
\newcommand{\bchi}{\bm{\chi}}
\newcommand{\bpsi}{\bm{\psi}}
\newcommand{\bomega}{\bm{\omega}}

\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bTheta}{\bm{\Theta}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bUpsilon}{\bm{\Upsilon}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bOmega}{\bm{\Omega}}


%----- Some standard definitions -----%

\newcommand{\independent}{\perp\!\!\!\!\perp}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\arginf} {\mathop{\mathrm{arginf}}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}}}

\newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\trace}{\mathop{\mathrm{Trace}}}

\DeclareMathOperator{\Var}{{\rm Var}}
\DeclareMathOperator{\Cor}{\rm Corr}
\DeclareMathOperator{\Cov}{\rm Cov}
\DeclareMathOperator{\ind}{\mathds{1}}  % Indicator
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}

\newcommand*{\zero}{{\bm 0}}
\newcommand*{\one}{{\bm 1}}

\newcommand{\diag}{{\rm diag}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%% Norms
\newcommand{\fro}{\mathop{\mathrm{fro}}}
\newcommand{\oper}{\mathop{\mathrm{op}}}

%%%%% Dot product
\newcommand{\dotp}[2]{\langle{#1},{#2}\rangle}

%%%%  brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}

%%%%%%%%%  Other commands

\newcommand{\mcomment}[1]{\marginpar{\tiny{#1}}}
\newcommand{\fcomment}[1]{\footnote{\tiny{#1}}}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\ud}{{\mathrm{d}}}


%%%%%%%%  amsmath %%%%%%%%%%
\newtheoremstyle{mytheoremstyle} % name
    {\topsep}                    % Space above
    {\topsep}                    % Space below
    {\normalfont}                   % Body font
    {}                           % Indent amount
    {\bfseries}                   % Theorem head font
    {.}                          % Punctuation after theorem head
    {.5em}                       % Space after theorem head
    {}  % Theorem head spec (can be left empty, meaning ‘normal’)

% \theoremstyle{mytheoremstyle}

% \ifx\BlackBox\undefined
% \newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
% \fi

% \ifx\QED\undefined
% \def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
% \fi

% \ifx\proof\undefined
% \newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
% %\newenvironment{proof}{\emph{Proof. }}{ \hfill \QED}
% \fi

% \ifx\theorem\undefined
% \newtheorem{theorem}{Theorem}[section]
% \fi
% \ifx\example\undefined
% %\newtheorem{example}[theorem]{Example}
% %\newtheorem{example}{Example}[section]
% \fi
% \ifx\property\undefined
% \newtheorem{property}{Property}[section]
% \fi
% \ifx\lemma\undefined
% %\newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{lemma}{Lemma}[section]
% \fi
% \ifx\proposition\undefined
% %\newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{proposition}{Proposition}[section]
% \fi
% \ifx\remark\undefined
% %\newtheorem{remark}[theorem]{Remark}
% \newtheorem{remark}{Remark}[section]
% \fi
% \ifx\corollary\undefined
% %\newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{corollary}{Corollary}[section]
% \fi
% \ifx\definition\undefined
% %\newtheorem{definition}[theorem]{Definition}
% \newtheorem{definition}{Definition}[section]
% \fi
% \ifx\conjecture\undefined
% %\newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{conjecture}{Conjecture}[section]
% \fi
% \ifx\fact\undefined
% %\newtheorem{fact}[theorem]{Fact}
% \newtheorem{fact}{Fact}[section]
% \fi
% \ifx\claim\undefined
% %\newtheorem{claim}[theorem]{Claim}
% \newtheorem{claim}{Claim}[section]
% \fi
% \ifx\assumption\undefined
% %\newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{assumption}{Assumption}[section]
% \fi
% \ifx\cond\undefined
% %\newtheorem{cond}[theorem]{Condition}
% \newtheorem{cond}{Condition}[section]
% \fi

% \newtheoremstyle{anothertheoremstyle} % name
%     {\topsep}                    % Space above
%     {\topsep}                    % Space below
%     {\normalfont}                   % Body font
%     {}                           % Indent amount
%     {\bfseries}                   % Theorem head font
%     {.}                          % Punctuation after theorem head
%     {.5em}                       % Space after theorem head
%     {\thmname{#1} \thmnumber{#2} \normalfont{#3}}  % Theorem head spec (can be left empty, meaning ‘normal’)
% \ifx\condition\undefined
% \theoremstyle{anothertheoremstyle}
% %\newtheorem{condition}[theorem]{Condition}
% \newtheorem{condition}{Condition}
% \fi
% \numberwithin{equation}{section}
% \numberwithin{theorem}{section}

% \makeatletter
% \newcommand{\raisemath}[1]{\mathpalette{\raisem@th{#1}}}
% \newcommand{\raisem@th}[3]{\raisebox{#1}{$#2#3$}}
% \makeatother

% \let\oldabstract\abstract
% \let\oldendabstract\endabstract
% \makeatletter
% \renewenvironment{abstract}
% {\renewenvironment{quotation}%
%                {\list{}{\addtolength{\leftmargin}{-0.5em} % change this value to add or remove length to the the default
%                        \listparindent 0em%
%                         \itemindent    \listparindent%
%                         \rightmargin   \leftmargin%
%                         \parsep        \z@ \@plus\p@}%
%                 \item\relax}%
%                {\endlist}%
% \oldabstract}
% {\oldendabstract}
% \makeatother

